Dual RL: Unification and New Methods for Reinforcement and Imitation Learning

The goal of reinforcement learning (RL) is to find a policy that maximizes the expected cumulative return. It has been shown that this objective can be represented as an optimization problem of state-action visitation distribution under linear constraints. The dual problem of this formulation, which we refer to as dual RL, is unconstrained and easier to optimize. In this work, we first cast several state-of-the-art offline RL and offline imitation learning (IL) algorithms as instances of dual RL approaches with shared structures. Such unification allows us to identify the root cause of the shortcomings of prior methods. For offline IL, our analysis shows that prior methods are based on a restrictive coverage assumption that greatly limits their performance in practice. To fix this limitation, we propose a new discriminator-free method ReCOIL that learns to imitate from arbitrary off-policy data to obtain near-expert performance. For offline RL, our analysis frames a recent offline RL method XQL in the dual framework, and we further propose a new method f-DVL that provides alternative choices to the Gumbel regression loss that fixes the known training instability issue of XQL. The performance improvements by both of our proposed methods, ReCOIL and f-DVL, in IL and RL are validated on an extensive suite of simulated robot locomotion and manipulation tasks. Project code and details can be found at this https://hari-sikchi.github.io/dual-rl.

==> 5method.tex <==
\section{Imitation Learning from Dual Perspective}
\label{sec:dual_imitation}


We consider the standard imitation learning setup where the agent is given a set of expert demonstrations, i.e. state-action trajectories, and does not have access to environment reward. We limit ourselves to the offline setup (no environment interactions allowed) in this work and discuss how the formulation extend to online setting under mild modifications in Appendix~\ref{}. We consider two possible offline IL settings --- where only expert demonstrations are available and the other where we additionally have access to suboptimal transitions from the environment. Intuitively, these suboptimal transitions should aid in better matching the expert behavior. For these two settings, we show in section~\ref{sec:connections_to_il} how prior work can be understood as dual-RL methods. Learning from expert demonstration along with access to suboptimal data is a ubiquitous problem in applications like robot learning and healthcare. Prior works in this setting solve this problem by learning a discriminator and using it for downstream offline RL. Errors in discriminator compound and lead to poor policy performance. Our analysis reveals that the root cause of needing to learn a discriminator is the coverage assumption, and propose a new discriminator-free method in section~\ref{sec:new_il_method} that eliminates these downsides. \looseness=-1

% Imitation learning is the setting where an agent does not have access to the reward when interacting with the environment.
% Instead, it is given a set of reward-free demonstrations, i.e. state-action trajectories. For ease of presentation, we start with the standard 
% \emph{offline IL} setup in Section~\ref{sec:connections_to_il}, where the demonstrations are generated by expert agents. We show how IQLearn~\cite{garg2021iq} and IBC~\cite{florence2022implicit} can be written as \dualQ problems. Next, we consider the setting in which the agents receive additional suboptimal demonstrations, where we rewrite OPOLO~\cite{zhu2020off} in the \dualQ formulation. Finally, we discuss how these formulations and algorithms further extend to \emph{online IL} under mild modifications. The process of unifying those algorithms helps us identify shortcomings and unprincipled components in them, and we propose a novel algorithm \texttt{ReCOIL} that eliminates those downsides in Section~\ref{sec:new_il_method}. \looseness=-1

\subsection{Dual Formulation for Existing Off-Policy Imitation Learning Algorithms}
\label{sec:connections_to_il}


\paragraph{Offline IL with Expert Data Only}
\label{main:offline_il_expert}

A straightforward application of our \dualQ formulation to offline IL is to simply set the reward to be uniformly $0$ across the state-action space and set the regularization distribution $d^O$ to be the expert visitation distribution $d^E$. That is,
% \colorbox{Goldenrod!30}{\texttt{dual-Q}~\text{(offline imitation with expert-only data)}}: 
\begin{equation}
\label{eq:dual-Q-imit}
\resizebox{0.92\textwidth}{!}{
    \colorbox{Goldenrod!30}{\dualQ}\,
    $\max_{\pi}\min_{Q} (1-\gamma)\E{d_0(s),\pi(a|s)}{Q(s,a)} +\alpha\E{s,a\sim d^E}{f^*\left(\left[\mathcal{T}^\pi_0 Q(s,a)-Q(s,a)\right]/
    \alpha\right)}$.
}
\end{equation}
Interestingly, this reduction directly leads us to a family of IL methods IQLearn~\citep{garg2021iq}, which was derived using a change of variables in the form of an inverse backup operator. 
% \qq{IQLearn also has an entropy regularizer $H(\pi)$, correspondingly the $Q$ learning update is different. need to have another soft-bellman operator}
\begin{restatable}[]{lemma}{iqlearn}
\label{lemma:iqlearn}
 IQLearn~\citep{garg2021iq} is an instance of $\texttt{dual-Q}$ using the semi-gradient update rule with a (soft) Bellman operator, where $r(s,a)=0 \, \forall s \in \mathcal{S}, a \in \mathcal{A}$, $d^O=d^E$.
 \vspace{-2mm}
\end{restatable}
%  We also find that IBC, an offline IL method that performs behavior cloning using a contrastive objective, is a special case of IQLearn and consequently of the \texttt{dual-Q} form.
% \begin{restatable}[]{corollary}{ibc}
% \label{corollary:ibc}
%  IBC~\citep{florence2022implicit} is an instance of \texttt{dual-Q} using the full-gradient update, where $r(s,a)=0~~\forall s \in \mathcal{S}, a \in \mathcal{A}$, $d^O=d^E$, and the $f$-divergence is the total variation distance. 
%  \vspace{-2mm}
% \end{restatable}

% \qq{I will move this sentence to Section 5.}
% The \texttt{dual-V} variant can be analogously leveraged to obtain a novel method for offline imitation learning, which we refer to as \texttt{IVLearn}. We leave this direction for future exploration and focus on the more general off-policy setting in this work. (See Appendix~\ref{ap:offline_imitation_learning_expert}).
\paragraph{Offline IL with Additional Suboptimal Data}
% \label{main:offpolicy_il_coverage}
The \texttt{dual-Q} and \texttt{dual-V} formulations do not naturally incorporate additional suboptimal data $d^S$. To remedy this, prior methods have relied on careful selection of the $f$-divergence and a \emph{coverage assumption} that allows them to craft an off-policy objective for imitation learning~\citep{zhu2020off,hoshino2022opirl,ma2022smodice,kim2022demodice,kim2022lobsdice}. More precisely, under the \emph{coverage assumption} that the suboptimal data visitation (denoted by $d^S$) covers the expert visitation ($d^S>0$ wherever $d^E>0$)~\citep{ma2022smodice}, and using the reverse KL divergence, we get the following objective:
\begin{align*}
  \kl{d(s,a)}{d^E(s,a)} &= \E{s,a\sim d(s,a)}{\log \frac{d(s,a)}{d^E(s,a)}}= \E{s,a\sim d(s,a)}{\log \frac{d(s,a)}{d^S(s,a)}+\log \frac{d^S(s,a)}{d^E(s,a)}}\\
  &= \E{s,a\sim d(s,a)}{\log \frac{d^S(s,a)}{d^E(s,a)}}+\kl{d(s,a)}{d^S(s,a)}.
\end{align*}
 This objective resembles \primalQ when $r(s,a)= - \log\tfrac{d^S(s,a)}{d^E(s,a)}$ and correspondingly we can get the following \dualQ problem using Eq.~\ref{eq:dual_q_original_equation}:
\begin{equation}
\label{eq:dual_q_il_coverage}
\resizebox{0.92\textwidth}{!}{
    \colorbox{Goldenrod!30}{\dualQ}\,
    $\max_{\pi(a|s)}\min_{Q(s,a)} (1-\gamma)\E{\rho_0(s),\pi(a|s)}{Q(s,a)}+\E{s,a\sim d^S}{f^*(\mathcal{T}^\pi_{r^{imit}}Q(s,a)-Q(s,a))}$,
}
\end{equation}
where $\Timit$ denote Bellman operator under the \emph{pseudo-reward} function $r^\text{imit}(s,a) = - \log\tfrac{d^S(s,a)}{d^E(s,a)}$. The pseudo-reward is precisely what is learned via a discriminator and then used for optimizing Equation~\ref{eq:dual_q_il_coverage}. Errors in learned discriminator can cascade for RL training and deteriorate the performance of output policy. This insight also allows us to reduce another IL method OPOLO~\citep{zhu2020off} to the \dualQ and defer the detailed discussion to Appendix~\ref{}. 
% This leads us to a reduction of another IL method OPOLO~\citep{zhu2020off} to \dualQ.
% \begin{restatable}[]{lemma}{opolo}
% OPOLO~\citep{zhu2020off} is an instance of $\texttt{dual-Q}$ using the semi-gradient update rule, where $r(s,a)=0~\forall \mathcal{S},\mathcal{A}$, $d^O=d^E$,
% and the $f$-divergence set to the reverse KL divergence.
% \vspace{-2mm}
% \end{restatable}



% We note that the \texttt{dual-V} framework for off-policy imitation learning under coverage assumptions with a full-gradient update rule was studied in SMODICE~\cite{ma2022smodice}.

% \textbf{From Offline to Online } Problem~\eqref{eq:dual_q_il_coverage} naturally extends to online IL, as the suboptimal data does not need to be static---it can be the replay buffer during online training. The corresponding algorithms generalize as well, since their key component is estimating the $Q^\pi$ function using \emph{off-policy} data. It is worth noting that $d^S$ is dynamically changing for online IL. In contrast, Eq.~\eqref{eq:dual-Q-imit} cannot be extended to online IL. \citet{garg2021iq} uses IQLearn in the online setting where they add additional regularization using bellman backups on $d^S$.
% Our results suggest this to be unprincipled (also pointed out by \citet{al2023ls}), as only expert data samples can be leveraged in this formulation. \looseness=-1


% b. for the latter case, as the suboptimal data is not necessarily static---it can be the replay buffer during online training. The corresponding algorithms generalize as well, since the key component of them is to estimate the $Q^\pi$ function using \emph{off-policy} data. \looseness=-1



% \subsection{Dual Formulations for Off-Policy Reinforcement Learning \hs{Variant 1}}  
% \label{sec:connections_to_rl}
% Regularized policy optimization (Eq.~\ref{eq:primal_rl_q_main} and~\ref{eq:primal_rl_v_main})
%  is a natural optimization objective for offline RL by preventing overestimation~\cite{liu2020provably,nair2020awac, fujimoto2019off}, and for online RL by improving convergence and training stability~\cite{schulman2015trust,kakade2001natural,sikchi2022learning}. Two notable frameworks for offline RL have seemingly been exceptions to the regularized policy optimization framework: Pessimistic value learning~\cite{kumar2020conservative} and Implicit Maximization based algorithms~\cite{garg2023extreme,kostrikov2021offline}. Our results below, first to our knowledge, combine all three classes together from the unified perspective of the dual RL framework, thus providing a simple justification for these methods while also paving the way to understanding which factors impact the performance of a method. Our experiments will explore this in the context of an implicit-maximization-based method~\cite{garg2023extreme}, whose superior performance was attributed to the property of Gumbel distribution better modeling bellman errors. Our first result formalizes the reduction of a popular family of pessimistic value learning methods -- Conservative Q learning~\citep{kumar2020conservative} to  \texttt{dual-Q}.
% \begin{restatable}[]{lemma}{cql}
% \label{thm:CQL}
% CQL is an instance of \dualQ where the generator function is $f(x)=(x-1)^2$ (corresponding to the Pearson $\chi^2$ divergence),
% and the regularization distribution $d^O$ is the offline visitation distribution.
% \end{restatable}
% % In other words, CQL eventually solves the same regularized policy optimization problem (\texttt{primal-Q}) as prior offline RL methods~\citep{nair2020awac,fujimoto2018addressing, wu2019behavior} in its dual form where the regularization is a particular form of $f$-divergence. 
% The above result indicates that its better performance compared to the family of behavior-regularized offline RL methods~\citep{nair2020awac,fujimoto2018addressing, wu2019behavior}, which solve the \texttt{primal-Q} using approximate dynamic programming is likely due to the choice of $f$-divergence and more amenable optimization afforded by the dual formulation. Notably, the \dualQ formulation has been previously studied for online RL in AlgaeDICE~\citep{nachum2019algaedice}. Lemma~\ref{thm:CQL} also suggests that CQL is an offline version of AlgaeDICE. 
%  
% Next, we show the \texttt{dual-V} framework leads to a family of implicit maximization methods for offline RL, thus tying in all three methods for offline RL - regularized policy optimization, pessimistic value learning, and implicit-value maximization based as instances of \texttt{primal-Q}, \texttt{dual-Q} and \texttt{dual-V} respectively.  We formalize the reduction of a recent implicit maximization-based method XQL to \texttt{dual-V} below.
% % Now we show that the \texttt{dual-V} framework leads to a family of implicit maximization methods, a special case of which is Extreme Q-Learning (XQL)~\citep{garg2023extreme}. We formalize the reduction of XQL to \texttt{dual-V} by considering a particular $f$-divergence and a semi-gradient update rule (i.e $\texttt{stop-gradient}\left(r(s,a)+\gamma \sum_{s'} p(s'|s,a)V(s')\right)$) in the lemma below.
% \begin{restatable}[]{lemma}{xql}
% \label{thm:XQL}
% XQL is an instance of \dualV where the generator function is $f(x) = x\log x$ (corresponding to reverse Kullback-Liebler divergence), the regularization distribution $d^O$ is the offline visitation distribution, and it uses a semi-gradient update rule (i.e $\texttt{stop-gradient}(\mathcal{T}V(s,a)$).
% \end{restatable}
% This insight behind lemma~\ref{thm:XQL} allows us to propose a class of algorithms extending XQL by choosing different generator functions,
% which result in a family of performant implicit policy improvement methods in Section~\ref{sec:new_rl_method}, and we show these methods enjoy better training stability in Section~\ref{sec:result}. \looseness=-1
% 
% Again, these offline methods naturally extend to online settings~\cite{kostrikov2021offline, garg2023extreme, nakamoto2023cal}, as their off-policy nature extends beyond the offline setup. The above results still hold, where the regularization distribution becomes the visitation distribution of the replay buffer $d^R$. It is worth noting that $d^R$ is dynamically changing over the course of training.


% We note that the \texttt{dual-V} framework for off-policy imitation learning under coverage assumptions was studied in the imitation learning work SMODICE~\citep{ma2022smodice}.

\subsection{\textbf{\texttt{ReCOIL}}: Imitation Learning from Arbitrary Experience}
\label{sec:new_il_method}



As demonstrated in Section~\ref{sec:connections_to_il},
previous off-policy IL methods often rely on the coverage assumption and train a discriminator between the demonstration and the offline data to obtain a pseudo-reward $r^\text{imit}$. 
We propose \textbf{RE}laxed \textbf{C}overage for \textbf{O}ff-policy \textbf{I}mitation \textbf{L}earning~(\texttt{ReCOIL}),
an off-policy IL algorithm that eliminates the need for both, the coverage assumption and consequently, the discriminator. To achieve this we consider matching mixture distributions which will provide us with an alternative way to leverage suboptimal data for imitation. Let $d_\text{mix}^S :=\beta d(s,a) + (1-\beta) d^S(s,a)$ and $d_\text{mix}^{E,S} := \beta d^E(s,a)+(1-\beta)d^S(s,a)$, where $\beta \in (0,1) $ is a fixed hyperparameter. We consider the following problem in \primalV form:
\begin{align}
\label{eq:primal_imitation_f_mixture}
\colorbox{RoyalBlue!15}{\primalQ} &~~~~~~~~~~~~~~~~~~~~~~~~~~~~\max_{d(s,a)} -\f{d^S_\text{mix}(s,a)}{d^{E,S}_\text{mix}(s,a)} \nonumber\\
   \text{s.t}~ \forall s \in \S, a\in \A,~~&\textstyle  d(s,a)=(1-\gamma)d_0(s)\pi(a|s)+\gamma \sum_{(s',a') \in \S \times \A } d(s',a') p(s|s',a') \pi(a|s)
\end{align}
This is a valid imitation learning formulation~\citep{ghasemipour2020divergence} since the global maximum of the objective is attained at $d=d^E$ which also satisfies the above constraints, irrespective of the suboptimal data distribution $d^S$. Finally, we derive the dual of the above objective in Lemma~\ref{thm:recoilq} which we term as \texttt{ReCOIL}. 

\begin{restatable}[]{lemma}{closerq}
\label{thm:recoilq}
(ReCOIL objective)The dual problem to the mixture distribution matching objective is given by:
\begin{equation}
   \resizebox{0.94\textwidth}{!}{ $\max_{\pi}\min_{Q}  \beta (1-\gamma)\E{d_0,\pi}{Q(s,a)} +\E{s,a\sim d_\text{mix}^{E,S}}{f^*_p(\mathcal{T}^{\pi}_0 Q(s,a )-Q(s,a))}  -(1-\beta) \E{s,a\sim d^S}{\mathcal{T}^{\pi}_0 Q(s,a )-Q(s,a)}$}
\end{equation}
and recovers the optimal policy $\pi^*$ as strong duality holds from Slater's conditions.
\end{restatable}


In other words, imitation learning can be solved by optimizing the unconstrained problem \texttt{ReCOIL-Q} with arbitrary off-policy data, without the coverage assumption. Besides, as opposed to many previous algorithms, \texttt{ReCOIL-Q} uses the Bellman operator $\mathcal{T}_0$ which does not need the pseudo-reward $r^\text{imit}$, therefore it is discriminator-free. Although the pseudo-reward is not needed for training, \texttt{ReCOIL-V} allows for recovering the reward function using the learned $V^*$ which corresponds to the intent of the expert. That is, $r(s,a)= V^*(s)-\mathcal{T}_0(V^*(s,a))$.
% and  $r(s,a)=Q^*(s,a)-\mathcal{T}^{\pi^*}_0(Q^*(s',a'))$ respectively. \looseness=-1
Moreover, our method is generic to incorporate any $f$-divergence.  The complete algorithm for \texttt{ReCOIL-V} can be found in Algorithm~\ref{algo:recoil_algorithm_idealized} in Appendix~\ref{ap:experiment_details}. 


\paragraph{A Bellman Consistent Energy-Based Model (EBM) View for ReCOIL}
Instantiating \texttt{ReCOIL-Q} with Pearson $\chi^2$ Divergence, we can simplify the objective (complete derivation in appendix~\ref{}) to:
\begin{equation}
\label{eq:recoil_intuition}
\resizebox{0.92\textwidth}{!}{
$\max_\pi \min_Q \beta (\E{d^S,\pi(a|s)}{Q(s,a)}-\E{d^E(s,a)}{Q(s,a)}) + \color{orange}
      \underbrace{\color{black}\E{s,a\sim \demix}{(\gamma Q(s',\pi(s'))-Q(s,a))^2}}_{\text{Bellman consistency}}$.
}
\end{equation}

One can see that \texttt{ReCOIL-Q} aims to learn a score function $Q$ whose expected value is low over the suboptimal distribution but high over the expert distribution, while ensuring that $Q$ is Bellman consistent over the mixture.
The Bellman consistency is crucial to propagate the information of how to recover when the policy makes a mistake. 
The $Q$ value can be interpreted as a score as it is not representative of any expected return, and we can view 
\texttt{ReCOIL-Q} as an energy-based model with Bellman consistency. Figure~\ref{fig:recoil_main} illustrates this intuition.
\looseness=-1

\paragraph{Practical Algorithm}: We consider three parameterized function $Q_\phi(s,a)$, $V_\theta(s)$ and $\pi_\psi$. Furthermore, we rely on Pearson $\chi^2$ divergence for ReCOIL (Eq.~\ref{eq:recoil_intuition}) as it has been shown to lead to stable learning for the imitation setting~\citep{garg2021iq}. Our practical algorithm uses a semi-gradient update that results in the training $Q_\phi$ as:
\begin{equation}
    \resizebox{0.92\textwidth}{!}{$ \mathcal{L}(\phi) = \beta (\E{d^S,\pi(a|s)}{Q_\phi(s,a)}-\E{d^E(s,a)}{Q_\phi(s,a)}) + \E{s,a\sim \demix}{(\gamma V_\psi(s')-Q_\phi(s,a))^2}$},
\end{equation}
 To prevent extrapolation error in the offline setting, we rely on an implicit maximizer (expectile regression from~\cite{kostrikov2021offline}) that pessimistically estimates the maximum of $Q(s,a)$ using in-distribution actions. 
\begin{equation}
    \mathcal{J}(\theta) =\E{s,a\sim \mathcal{D}}{L^\tau_2(V_\theta(s,g)-Q_\phi(s,a))},
\end{equation}
where $L^\tau_2(u)=|\tau-1(u<0)|u^2$. Finally, the policy is extracted via advantage-weighted regression~\citep{}. Algorithm~\ref{} details the implementation.
\begin{equation}
    \mathcal{M}(\psi) =\max_\psi \E{s,a\sim d^O}{\text{exp}(\tau (Q_\phi(s,a)-V_\theta(s))) \log(\pi_\theta(a|s))},
\end{equation}. 



\section{Reinforcement Learning from Dual Perspective}



\label{sec:dual_reinforcement}
Regularized policy optimization, in its various forms~\citep{fujimoto2019off, wu2019behavior}, is a natural objective for off-policy algorithms, in both offline and online settings.
In offline RL, various types of conservatism notions have been proposed to prevent overestimated $Q$-values~\citep{fu2019diagnosing}. A performant notion of conservatism is implicit policy improvement (XQL~\citep{garg2023extreme}), which uses in-distribution samples to pessimistically estimate the greedy improvement to the $Q$-function. Lemma~\ref{thm:XQL} shows, perhaps surprisingly, that XQL can be cast as a \dualV problem.


\begin{restatable}[]{lemma}{xql}
\label{thm:XQL}
XQL is an instance of \dualV under the semi-gradient update rule,
where the $f$-divergence is the reverse Kullback-Liebler divergence,
and $d^O$ is the offline visitation distribution. 
\vspace{-2mm}
\end{restatable}
The success of XQL was attributed to the property that Gumbel distribution better models the Bellman errors~\citep{garg2023extreme}. Despite its decent performance, XQL is prone to training instability (see e.g., Figure~\ref{fig:offline-rl-analysis}), since the Gumbel loss is an exponential function that can produce large gradient during training. 
% Two notable frameworks for offline RL are pessimistic value learning 
% e.g. CQL~\citep{kumar2020conservative} and implicit policy improvement algorithms including IQL~\citep{kostrikov2021offline} and XQL~\citep{garg2023extreme}. These frameworks have seemingly been exceptions to the regularized policy optimization formulation (Eq.~\eqref{eq:primal_rl_q_main} and~\eqref{eq:primal_rl_v_main}). Nonetheless, our results in Section~\ref{sec:connections_to_rl}, first to our knowledge, formulate both of them as instances of dual-RL, and thus solving regularized policy optimization in essence. Such unification also allows us to propose \textbf{$f$-DVL}, a new offline RL method under this framework in Section~\ref{sec:new_rl_method}. 


% \subsection{Dual Formulations for Existing Off-Policy Reinforcement Learning Algorithms} % \hs{Variant 2}}
% \label{sec:connections_to_rl}

% Our first result, perhaps surprisingly, places a class of pessimistic value learning methods, CQL, as a dual-RL method with a particular choice of $f$-divergence. 
% \begin{restatable}[]{lemma}{cql}
% \label{thm:CQL}
% CQL is an instance of \dualQ under the semi-gradient update rule, where the $f$-divergence is the Pearson $\chi^2$ divergence,
% and $d^O$ is the offline visitation distribution. 
% \vspace{-2mm}
% \end{restatable}

% Next, we show that \dualV subsumes a family of implicit policy improvement methods for offline RL, thus tying together all three types of methods -- policy regularized, pessimistic value function, and implicit maximization based as instances of \primalQ, \dualQ and \dualV respectively. We formalize the reduction of XQL, a recent implicit policy improvement method, to \dualV below.

% \begin{restatable}[]{lemma}{xql}
% \label{thm:XQL}
% XQL is an instance of \dualV under the semi-gradient update rule,
% %(i.e $\texttt{stop-gradient}(\mathcal{T}_rV(s,a)$),
% where the $f$-divergence is the reverse Kullback-Liebler divergence,
% % ($f^*(y) = e^{y-1}$), 
% and $d^O$ is the offline visitation distribution. 
% \vspace{-2mm}
% \end{restatable}

\subsection{\textbf{\texttt{$f$-DVL}} (Dual-V Learning): Better Implicit Maximizers for Offline RL}
\label{sec:new_rl_method}
Lemma~\ref{thm:XQL} shows that XQL is a particular \dualV problem where the Gumbel loss is the conjugate $f^*_p$ corresponding to reverse KL divergence. This insight allows us to extend XQL by choosing different $f$-divergences, where the conjugate functions are more optimization amenable. We further show that the proposed methods enjoy both improved performance and better training stability in Section~\ref{sec:result}. \looseness=-1


Implicit policy improvement algorithms iterate two steps alternately: 1) regress $Q(s,a)$ to $r(s,a)+\gamma V(s')$ for transition $(s, a, s')$, 2) estimate $V(s) = \max_{a \in A} Q(s,a)$. The learned $Q$, $V$ functions can be used to extract policy as for the \dualV formulation, see Appendix~\ref{ap:recovering_policy}. Step 1) is akin to the \emph{policy evaluation} step of generalized policy iteration (GPI), and step 2) acts like the \emph{policy improvement} step without explicitly learning a policy $\pi(s) = \argmax_a Q(s,a)$. The crux is to conservatively estimate the maximum of $Q$ in step 2.
\looseness=-1

Consider a rewriting of \dualV with the temperature parameter $\lambda$: 
\begin{equation}
\label{eq:implicit_maximization}
    \min_{V} (1-\lambda)\E{s \sim d^O}{V(s)} +\lambda\E{(s,a)\sim d^O}{
    f^*_p\left(\bar{Q}(s,a)-V(s)\right)},
\end{equation}
where $\bar{Q}(s,a)$ denotes $\texttt{stop-gradient}(r(s,a)+\gamma \sum_{s'} p(s'|s,a)V(s'))$. 
Let $x$ be a random variable of distribution $D$. Eq~\eqref{eq:implicit_maximization} can be considered as a special instance of the following problem:\looseness=-1
% Eq~\ref{eq:implicit_maximization} can be rewritten as:
\begin{equation}
\label{eq:implicit_maximization_general}
\min_{v} (1-\lambda) v + \lambda\E{x\sim D}{f^*_p\left( x-v  \right)},
\end{equation}
where $x$ is analogous to $\bar{Q}$ and $v$ is analogous to $V$. As opposed to the handcrafted choices~\citep{kostrikov2021offline, garg2023extreme},
we show through Lemma~\ref{thm:implicit_maximizer} below that problem~\eqref{eq:implicit_maximization_general}
% the \dualV formulation 
naturally gives rise to a family of \emph{implicit maximizers} that estimates $\sup_{x \sim D} x$ as $\lambda \rightarrow 1$,.

% Intuitively, this is because the second term in Eq~\ref{eq:implicit_maximization_general} is minimized in value as $v$ increases and saturates once $v=\max (x\in support(D))$ while the first term is minimized for smaller $v$.  
\begin{restatable}[]{lemma}{implicit}
\label{thm:implicit_maximizer}
Let $x$ be a real-valued random variable such that $\Pr(x > x^*) = 0$.
% whose supremum is $x^*$. 
Let $v_\lambda$ be the solution of Problem~\eqref{eq:implicit_maximization_general}. It holds that $v_{\lambda_1}\le v_{\lambda_2}$, $\forall \, 0 < \lambda_1  < \lambda_2 < 1$. Further,
%\begin{equation}
$\lim_{\lambda\to 1} v_\lambda = x^*$.
%\end{equation}
\end{restatable}
 Figure~\ref{fig:implicit_maximizers} shows an illustration for Lemma~\ref{thm:implicit_maximizer}. We propose a family of maximizers associated with different $f$-divergences and apply them to \dualV. We call the resulting methods $f$-\texttt{DVL} (Dual-V Learning).
 
 \paragraph{Practical considerations and algorithm}: A practical issue in optimizing Eq~\ref{eq:implicit_maximization} is that $f^*_p$ is not well defined over the entire domain of $\mathbb{R}$. To remedy this we consider an extension of $f^*_p$ in the form of the surrogates denoted by $\bar{f^*_p}$: for (1) Total Variation: $f(x) = \tfrac{1}{2}|x - 1|,   \bar{f^*_p}(y) = \max(y, 0)$, (2) Pearson $\chi^2$ divergence: $f(x) = (x-1)^2, \; \bar{f^*_p}(y) = \max(\tfrac{1}{4}y^2 + y, 0)$. We defer the derivation of these surrogates to Appendix~\ref{}. Recall that XQL uses the implicit maximizer associated with reverse KL divergence where $f^*_p$ is exponential. Compared with XQL, our $f^*_p$ functions are low-order polynomials and are thus stable for optimization. Algorithm~\ref{algo:dvl_algorithm} details the steps for \texttt{$f$-DVL}.
\looseness=-1
% two of which we consider here: 
% total variation (TV) and Pearson $\chi^2$ divergences \qq{discuss switing to presenting $f$ directly, and the zero thing.}:
% \begin{equation*}
%     \begin{aligned}
%     \text{(1) Total Variation:} \quad & f(x) = \tfrac{1}{2}|x - 1|, \;  f^*_p(y) = \max(y, 0) , \\ % \min_{v} (1-\lambda)\E{x\sim D}{v}+ \lambda\E{x\sim D}{\max(x-v,0)}, \\
%      \text{(2) Pearson $\chi^2$ divergence:} \quad &  f(x) = (x-1)^2, \; f^*_p(y) = \max(\tfrac{1}{4}y^2 + y, 0).% \min_{v} (1-\lambda)\E{x\sim D}{v}+ \lambda\E{x\sim D}{\max((x-v)+ 0.5(x-v)^2,0)}.
% \end{aligned}
% \end{equation*}
% See Figure~\ref{fig:implicit_maximizers} for an illustration. Compared with XQL, our $f^*_p$ functions are low-order polynomials and are thus stable for optimization. 

% We further show that the proposed methods enjoy both improved performance and better training stability in Section~\ref{sec:result}. \looseness=-1

% \qq{I moved this sentence to Section 4.3.} We also highlight that the full-gradient variant of the \texttt{dual-V} framework for offline RL has been studied extensively in OptiDICE~\citep{lee2021optidice}.

% \textbf{A family of implicit maximizers}: 
% Consider the $\lambda$-parameterized semi-gradient \dualV objective:
% \begin{equation}
% \label{eq:implicit_maximization}
%     \min_{V} (1-\lambda)\E{s \sim d^O}{V(s)} +\lambda\E{(s,a)\sim d^O}{
%     f^*_p\left(\bar{Q}(s,a)-V(s)\right)},
% \end{equation}
% where $\bar{Q}(s,a)$ denotes the target $Q$ value $\texttt{stop-gradient}(r(s,a)+\gamma \sum_{s'} p(s'|s,a)V(s'))$. 


% More generally,
% for any random variable $X$ with distribution $D$, Eq~\ref{eq:implicit_maximization} can be rewritten as:
% \begin{equation}
% \label{eq:implicit_maximization_general}
% \min_{v} (1-\lambda)\E{x\sim D}{v}+ \lambda\E{x\sim D}{f^*_p\left( x-v  \right)}.
% \end{equation}
% We show through Lemma~\ref{thm:implicit_maximizer} below and a simple example~\ref{fig:implicit_maximizers} that the semi-gradient form of \texttt{dual-V} optimization naturally gives rise to a family of implicit maximizers. Intuitively, this is because the second term in Eq~\ref{eq:implicit_maximization_general} is minimized in value as $v$ increases and saturates once $v=\max (x\in support(D))$ while the first term is minimized for smaller $v$.  This is opposed to specially curated implicit maximizers found in offline RL methods~\citep{kostrikov2021offline}. 
% For our experiments, we focus on the two implicit maximizers obtained using TV and $\chi^2$ divergences shown below:
% \begin{align}
%     \text{TV:}& \min_{v} (1-\lambda)\E{x\sim D}{v}+ \lambda\E{x\sim D}{\max(x-v,0)}.\\
%      \text{$\chi^2$:}& \min_{v} (1-\lambda)\E{x\sim D}{v}+ \lambda\E{x\sim D}{\max((x-v)+ 0.5(x-v)^2,0)}.
% \end{align}
% The complete algorithm for XQL++ can be found in Appendix~\ref{ap:xql++algorithm_implementation}. We also highlight that the full-gradient variant of the \texttt{dual-V} framework for offline RL has been studied extensively in OptiDICE~\citep{lee2021optidice}.
% We show in a simple example (Figure ~\ref{fig:implicit_maximizers}) that the semi-gradient form of \texttt{dual-V} optimization naturally gives rise to a family of implicit maximizers (estimators for extreme values of the distribution). 
% %%AZ.2.8: What is the start of the sentence to the objective below?
% This is opposed to specially curated implicit maximizers found in offline RL methods~\citep{kostrikov2021offline}. XQL's Gumbel regression is an implicit maximizer in the proposed family arising from the \texttt{dual-V} form for reverse KL divergence. We can potentially enjoy better optimization and convergence by choosing different $f$-divergences for dual-value function updates corresponding to different divergences. We list some of the loss functions for value function updates with different $f$-divergences in Appendix~\ref{ap:implicit_maximizers_family}. We also highlight that the full-gradient variant of the dual-V framework for offline RL has been studied extensively in OptiDICE~\citep{lee2021optidice}.
%%AZ.1.27: Could be good to include a table of dual offline/online RL methods and their differences. 
% \begin{restatable}[]{lemma}{implicit}
% \label{thm:implicit_maximizer}
% Let $X$ be a real-valued random variable with bounded support and the supremum of the support is $x^*$. Then optimizing equation~\ref{eq:implicit_maximization_general}, the solution $v_\lambda$ satisfies the following properties
% \begin{equation}
%     \lim_{\lambda\to 1} v_\lambda = x^* ~\text{and}~ \forall ~\lambda_1<\lambda_2 \in (0,1),~~v_{\lambda_1}\le v_{\lambda_2}.
% \end{equation}
% \end{restatable}
%%AZ.3.8: Explain in text why the reader should care about this lemma
% \proof{Refer Appendix}
% \textbf{A generalized policy iteration view of semi-gradient \texttt{dual-V}: } \hs{push to appendix\texttt{dual-V} framework presents optimization difficulties when using full-gradients~\citep{dai2017boosting}. X-QL shows that stable learning can be achieved using the semi-gradient form.} Our insight into implicit maximizers suggests that using semi-gradients brings the \texttt{dual-V} framework closer to generalized policy-iteration (GPI) framework. The update of $V$ in its semi-gradient dual form acts as an implicit policy optimizer and the estimation of $\hat{Q}(s,a)$ by regressing to $r(s,a)+\gamma V(s')$ is akin to a policy evaluation step, bridging the connection to GPI.



==> 6experiments-old.tex <==
% \vspace{-5mm}
\section{Experiments}
% \vspace{-2mm}
\label{sec:result}
% Due to We focus on offline IL and offline RL.
% Our experiments aim to answer the following questions: ....


\subsection{Offline IL}
\textbf{Benchmark and Analysis.}
Our experiments benchmark the performance of ReCOIL on an extensive set of 26 tasks with 9 simulated robots. We consider the offline setup to test ReCOIL's ability to imitate experts, decoupled from exploration difficulties. The offline suboptimal $d^S$ and expert datasets $d^E$ are obtained from the D4RL benchmark~\citep{fu2020d4rl}. Across all tasks, our agent is given access to 1 expert demonstration aside from the suboptimal transition dataset. More information on the suboptimal dataset composition can be found in Appendix~\ref{ap:offline_il_experiment_details}. We compare ReCOIL against recent methods specifically designed for the offline imitation setup -- RCE~\citep{eysenbach2021replacing}, SMODICE~\citep{ma2022smodice} and ORIL~\citep{zolna2020offline}. RCE is the SOTA example-based RL method and ORIL learns a state-action discriminator. RCE and ORIL use TD3-BC~\cite{fujimoto2021minimalist} to cope with the offline setup. SMODICE is a dual imitation method built on the coverage assumption. We do not compare to DEMODICE~\citep{kim2022demodice} as SMODICE was shown to be competitive in ~\cite{ma2022smodice}.

% In this task, we use an offline dataset of environment interactions from D4RL~\citep{fu2020d4rl}. We consider the following MuJoCo environments: Hopper, Walker2d, HalfCheetah, and Ant. We consider three different dataset compositions for the offline dataset - `random+expert', `medium+expert', and `random+few-expert'. The first two datasets consist of a few expert trajectories ($\le$200) and a large number of suboptimal transitions (1 million). random+few-expert has only $\le 30$ expert trajectories. The learning agent also has access to 1000 expert transitions. We compare recent methods for offline imitation learning with suboptimal data -- RCE~\citep{eysenbach2021replacing}, SMODICE~\citep{ma2022smodice} and ORIL~\citep{zolna2020offline}. We do not compare to DEMODICE~\citep{kim2022demodice} as SMODICE was shown to be competitive in ~\cite{ma2022smodice}.

% Our dataset composition is similar to SMODICE~\citep{ma2022smodice} where we use a mixture of a small number of expert trajectories ($\le$ 200 trajectories) and a large number of low-quality trajectories from the “random-v2” dataset (1 million transitions). We compare recent methods for offline imitation learning with suboptimal data -- SMODICE~\citep{ma2022smodice} and ORIL~\citep{zolna2020offline}. We do not compare to DEMODICE~\citep{kim2022demodice} as SMODICE was shown to be competitive in ~\cite{ma2022smodice}.

\begin{table*}[t]
\label{table:offline_il_results} 
    \scriptsize
    % \setlength\tabcolsep{3pt}
    \centering
    \begin{tabular}{c|c|c|c|c|c}
    \toprule
    \multirow{1}{*}{Dataset} & Env & RCE & ORIL & SMODICE & \texttt{ReCOIL}  \\
    \midrule
    \multirow{2}{*}{random+}& hopper&51.41$\pm$38.63&73.93$\pm$11.06&{101.61$\pm$7.69}&\highlight{108.18$\pm$3.28}\\
    & halfcheetah&64.19$\pm$11.06&60.49$\pm$3.53& 80.16$\pm$7.30&\highlight{80.20$\pm$6.61}\\
    \multirow{1}{*}{expert}& walker2d&20.90$\pm$26.80&2.86$\pm$3.39&\highlight{105.86$\pm$3.47}&102.16$\pm$7.19\\
    & ant&105.38$\pm$14.15&73.67$\pm$12.69&\highlight{126.78$\pm$5.12}&\highlight{126.74$\pm$4.63}\\
    \midrule
        \multirow{2}{*}{random+}& hopper&25.31$\pm$18.97&42.04$\pm$13.76&60.11$\pm$18.28&\highlight{97.85$\pm$17.89}\\
    & halfcheetah& 2.99$\pm$1.07&2.84$\pm$5.52& 2.28$\pm$0.62& \highlight{76.92$\pm$7.53}\\
    \multirow{1}{*}{few-expert}& walker2d&40.49$\pm$26.52& 3.22$\pm$3.29&\highlight{107.18$\pm$1.87}&83.23$\pm$19.00\\
    & ant&\highlight{67.62$\pm$15.81}&25.41 $\pm$ 8.58&-6.10$\pm$7.85&\highlight{67.14$\pm$ 8.30}\\
    \midrule
    \multirow{2}{*}{medium+}& hopper&58.71$\pm$34.06&61.68$\pm$7.61&49.74$\pm$3.62&\highlight{88.51$\pm$16.73}\\
    & halfcheetah&65.14$\pm$13.82& 54.66$\pm$0.88&59.50$\pm$0.82&\highlight{81.15$\pm$2.84}\\
    \multirow{1}{*}{expert}& walker2d&96.24$\pm$14.04&8.19$\pm$7.70&2.62$\pm$0.93&\highlight{108.54$\pm$1.81}\\
    & ant&86.14$\pm$38.59&102.74$\pm$6.63&104.95$\pm$6.43&\highlight{120.36$\pm$7.67} \\
    \midrule
    \multirow{2}{*}{medium}& hopper&66.15$\pm$35.16&17.40$\pm$15.15&47.61$\pm$7.08&\highlight{50.01$\pm$10.36}\\
    & halfcheetah&61.14$\pm$18.31& 43.24$\pm$0.75&46.45$\pm$3.12&\highlight{$\pm$\qq{missing?}}\\
    \multirow{1}{*}{few-expert}& walker2d&$\pm$\qq{missing?}&6.81$\pm$6.76&6.00$\pm$6.69&\highlight{91.25$\pm$17.63}\\
    & ant&67.95$\pm$36.78&81.53$\pm$8.618&81.53$\pm$8.618&\highlight{110.38$\pm$10.96} \\
    \midrule
    \multirow{4}{*}{cloned+expert}& pen&19.60$\pm$11.40&-3.10$\pm$0.40&-3.36$\pm$0.71&95.04$\pm$4.48\\
    & door&0.08$\pm$ 0.15&-0.33$\pm$0.01& 0.25$\pm$ 0.54&\highlight{102.75$\pm$4.05}\\
    & hammer&1.95$\pm$3.89&0.25$\pm$ 0.01&0.15$\pm$ 0.078&95.77$\pm$17.90\\
    & relocate&-0.25$\pm$0.04&-0.29$\pm$0.01&1.75$\pm$3.85&\highlight{67.43$\pm$14.60}\\
    \midrule
        \multirow{4}{*}{human+expert}& pen&17.81$\pm$5.91&-3.38$\pm$2.29&-2.20$\pm$2.40&\highlight{103.72$\pm$2.90}\\
    & door& -0.05$\pm$0.05&-0.33$\pm$0.01& -0.20$\pm$ 0.11& \highlight{104.70$\pm$0.55}\\
    & hammer&5.00$\pm$5.64& 1.89$\pm$0.70&-0.07$\pm$0.39&125.19$\pm$3.29\\
    & relocate&0.02$\pm$0.10& -0.29$\pm$0.01 &-0.16$\pm$0.04&\highlight{91.98$\pm$ 2.89}\\
    \midrule
    \multirow{1}{*}{partial+expert}& kitchen&6.875$\pm$9.24&0.00$\pm$0.00&39.16$\pm$ 1.17&\highlight{60.0$\pm$5.70}\\
    \midrule
    \multirow{1}{*}{mixed+expert}& 
    kitchen&1.66$\pm$2.35& 0.00$\pm$0.00&42.5$\pm$2.04&\highlight{52.0$\pm$1.0}\\
    \bottomrule
    \end{tabular}
\caption{The normalized return obtained by different offline IL methods, trained on the D4RL suboptimal datasets with 
1000 expert transitions. \texttt{ReCOIL} outperforms the others, both when the offline dataset has low coverage of the expert data, and when it is challenging to distinguish the expert transitions from the suboptimal ones. Each result is an average over 7 random seeds.} 
\end{table*}

\begin{wrapfigure}{r}{0.4\textwidth}
\begin{center}
% \vspace{-5pt}
\includegraphics[width=1.0\linewidth]{figures/rewards/reward_didactic.pdf}
\end{center}
\vspace{-4.5mm}
\caption{Recovered $R$ and $V^*$ on a simple continuous gridworld environment by \texttt{ReCOIL}.}
\label{fig:recovering_rewards}
\end{wrapfigure}

We focus on \texttt{ReCOIL-V} due to its favorable property of being a single-player non-adversarial optimization. Note, that contrary to SMODICE~\citep{ma2022smodice} which is based on the coverage assumption and requires learning a discriminator, \texttt{ReCOIL} directly learns the $V$ function. 
\begin{wrapfigure}{r}{0.6\textwidth}
\begin{center}
% \vspace{-20pt}
\includegraphics[width=1.0\linewidth]{figures/density_ratio_estimation/perfect_coverage_1d.pdf}
    \vspace{-7.5mm}
\end{center}
\caption{The replay buffer distribution covers the agent policy visitation distribution. Using \texttt{ReCOIL}, we are perfectly able to infer the agent policy visitation whereas a method that only relies on expert data or the replay data with the coverage assumption fails. Results are averaged over 100 seeds.}
\label{fig:distribution_ratio_estimation1}
% \vspace{-0.8mm}
\end{wrapfigure}Table~\ref{table:offline_il_results} empirically validate that \texttt{ReCOIL} strongly outperforms baselines in most environments. SMODICE shows poor performance in cases when the combined offline dataset has low expert coverage (random+few-expert) or where the discriminator can easily overfit (high-dimensional environments like dextrous manipulation). 

\textbf{Recovered Rewards}: Figure~\ref{fig:recovering_rewards} shows an example of a recovered reward function for a simple continuous grid-world task. We observe a Pearson correlation of \textbf{0.98} and \textbf{0.92} for Hopper and Walker recovered reward function with ground truth rewards. More details can be found in Appendix~\ref{ap:recovering_rewards}.



% \begin{table*}[t]
%     % \vspace{2mm}
%     % \centering
%     \tiny
%     % \setlength\tabcolsep{3pt}
%     \begin{minipage}[c]{.46\textwidth}
%     \centering
%     \resizebox{1.0\linewidth}{!}{%
%     \begin{tabular}{c|c|c|c|c|c}
%     \toprule
%     \multirow{1}{*}{Dataset} & Env & RCE & ORIL & SMODICE & \texttt{ReCOIL}  \\
%     \midrule
%     \multirow{2}{*}{random+}& hopper&51.41&73.93&{101.61}&\highlight{108.18}\\
%     & halfcheetah&64.19&60.49& 80.16&\highlight{80.20}\\
%     \multirow{1}{*}{expert}& walker2d&20.90&2.86&\highlight{105.86}&102.16\\
%     & ant&105.38&73.67&\highlight{126.78}&\highlight{126.74}\\
%     \midrule
%         \multirow{2}{*}{random+}& hopper&25.31&42.04&60.11&\highlight{97.85}\\
%     & halfcheetah& 2.99&2.84& 2.28& \highlight{76.92}\\
%     \multirow{1}{*}{few-expert}& walker2d&40.49& 3.22&\highlight{107.18}&83.23\\
%     & ant&\highlight{67.62}&25.41 &-6.10&\highlight{67.14}\\
%     \midrule
%     \multirow{2}{*}{medium+}& hopper&58.71&61.68&49.74&\highlight{88.51}\\
%     & halfcheetah&65.14& 54.66&59.50&\highlight{81.15}\\
%     \multirow{1}{*}{expert}& walker2d&96.24&8.19&2.62&\highlight{108.54}\\
%     & ant&86.14&102.74&104.95&\highlight{120.36} \\
%     \bottomrule
%     \end{tabular}}
% % \caption{Normalized scores for \texttt{ReCOIL} on the different D4RL datasets along with 1000 given expert transitions compared to different offline IL baselines. \texttt{ReCOIL} improves over baselines when the offline dataset has low coverage of expert or when it is more challenging to distinguish expert vs suboptimal transitions. } 
% \label{table:offline_il_results1}
% \end{minipage}
% \hskip0.02\textwidth
% \begin{minipage}[c]{0.52\textwidth}
% \resizebox{1.0\linewidth}{!}{%
%     \begin{tabular}{c|c|c|c|c|c}
%     \toprule
%     \multirow{1}{*}{Dataset} & Env & RCE & ORIL & SMODICE & \texttt{ReCOIL}  \\
%     \midrule
%     \multirow{2}{*}{medium}& hopper&66.15&17.40&47.61&\highlight{50.01}\\
%     & halfcheetah&61.14& 43.24&46.45&\highlight{$\pm$\qq{missing?}}\\
%     \multirow{1}{*}{few-expert}& walker2d&$\pm$\qq{missing?}&6.81&6.00&\highlight{91.25}\\
%     & ant&67.95&81.53&81.52&\highlight{110.38} \\
%     \midrule
%     \multirow{4}{*}{cloned+expert}& pen&19.60&-3.10&-3.36&95.04\\
%     & door&0.08&-0.33& 0.25&\highlight{102.75}\\
%     & hammer&1.95&0.25&0.15&95.77\\
%     & relocate&-0.25&-0.29&1.75&\highlight{67.43}\\
%     \midrule
%         \multirow{4}{*}{human+expert}& pen&17.81&-3.38&-2.20&\highlight{103.72}\\
%     & door& -0.05&-0.33& -0.20& \highlight{104.70}\\
%     & hammer&5.00& 1.89&-0.07&125.19\\
%     & relocate&0.02& -0.29 &-0.16&\highlight{91.98}\\
%     \midrule
%     \multirow{1}{*}{partial+expert}& kitchen&6.875&0.00&39.16&\highlight{60.0}\\
%     \midrule
%     \multirow{1}{*}{mixed+expert}& 
%     kitchen&1.66& 0.00&42.5&\highlight{52.0}\\
%     \bottomrule
%     \end{tabular}
% }

% \label{table:offline_il_results2} 
% \end{minipage}
% % \caption{Normalized scores for \texttt{ReCOIL} on the different D4RL datasets along with 1000 given expert transitions compared to different offline IL baselines. \texttt{ReCOIL} improves over baselines when the offline dataset has low coverage of expert or when it is more challenging to distinguish expert vs suboptimal transitions. } 
% \caption{The normalized return obtained by different offline IL methods, trained on the D4RL datasets with additional 
% 1000 expert transitions. \texttt{ReCOIL} outperforms the others, both when the offline dataset has low coverage of the expert data, and when it is challenging to distinguish the expert transitions from the suboptimal ones.} 
% \end{table*}


% #-------------------




% \begin{table*}[h]
%     % \vspace{2mm}
%     \centering
%     \scriptsize
%     % \resizebox{\textwidth}{!}{%
%     \begin{tabular}{c|c|c|c|c|c}
%     \toprule
%     \multirow{1}{*}{Dataset} & Env & RCE & ORIL & SMODICE & \texttt{ReCOIL}  \\
%     \midrule
%     \multirow{4}{*}{cloned+expert}& pen&19.60$\pm$11.40&-3.10$\pm$0.40&-3.36$\pm$0.71&95.04$\pm$4.48\\
%     & door&0.08$\pm$ 0.15&-0.33$\pm$0.01& 0.25$\pm$ 0.54&\textbf{102.75$\pm$4.05}\\
%     & hammer&1.95$\pm$3.89&0.25$\pm$ 0.01&0.15$\pm$ 0.078&95.77$\pm$17.90\\
%     & relocate&-0.25$\pm$0.04&-0.29$\pm$0.01&1.75$\pm$3.85&\textbf{67.43$\pm$14.60}\\
%     \midrule
%         \multirow{4}{*}{human+expert}& pen&17.81$\pm$5.91&-3.38$\pm$2.29&-2.20$\pm$2.40&\textbf{103.72$\pm$2.90}\\
%     & door& -0.05$\pm$0.05&-0.33$\pm$0.01& -0.20$\pm$ 0.11& \textbf{104.70$\pm$0.55}\\
%     & hammer&5.00$\pm$5.64& 1.89$\pm$0.70&-0.07$\pm$0.39&125.19$\pm$3.29\\
%     & relocate&0.02$\pm$0.10& -0.29$\pm$0.01 &-0.16$\pm$0.04&\textbf{91.98$\pm$ 2.89}\\
%     \midrule
%     \multirow{1}{*}{partial+expert}& kitchen&6.875$\pm$9.24&0.00$\pm$0.00&39.16$\pm$ 1.17&\textbf{60.0$\pm$5.70}\\
%     \midrule
%     \multirow{1}{*}{mixed+expert}& 
%     kitchen&1.66$\pm$2.35& 0.00$\pm$0.00&42.5$\pm$2.04&\textbf{52.0$\pm$1.0}\\
%     \bottomrule
%     \end{tabular}
% \caption{Normalized scores for \texttt{ReCOIL} on the different D4RL datasets along with 1000 given expert transitions compared to different offline IL baselines. \texttt{ReCOIL} improves over baselines when the offline dataset has low coverage of expert or when it is more challenging to distinguish expert vs suboptimal transitions. } 
% \label{table:offline_il_results2}
% \end{table*}

\textbf{Offline IL Analysis: Does \texttt{ReCOIL} allow for better estimation of the agent visitation distribution?}



% \begin{figure}[h]
% \begin{center}
% \includegraphics[width=0.5\linewidth]{figures/density_ratio_estimation/perfect_coverage_1d.pdf}
%       \\
%       \vspace{-2.0mm}
% \end{center}
% % \vspace{-1.0mm}
% \caption{The replay buffer distribution covers the agent policy visitation distribution. Using \texttt{ReCOIL}, we are perfectly able to infer the agent policy visitation whereas a method that only relies on expert data or the replay data with the coverage assumption fails. Results are averaged over 100 seeds.}
% \label{fig:distribution_ratio_estimation1}
% \end{figure}

\hs{For dual algorithms like \texttt{ReCOIL}, optimizing Eq~\ref{eq:dual-Q-inner} captures the fixed policy's visitation distribution in the first derivative of conjugate $f$-divergence (Sec.~\ref{sec:dual_rl})}. Estimating a policy's visitation correctly is key to testing its closeness to the expert visitation and in turn, solving the imitation learning problem. We show through experiments in Figure~\ref{fig:distribution_ratio_estimation1} and Figure~\ref{fig:distribution_ratio_estimation2} that ReCOIL is able to leverage the off-policy data to aid in recovering the given policy's visitation more accurately than methods that only utilize the expert data~\cite{garg2021iq} or those which use the off-policy data but under a coverage assumption~\cite{ma2022smodice,zhu2020off}. This validates our theoretical results in Theorem~\ref{thm:recoil}.

% We consider the proposed \texttt{ReCOIL} method and investigate its ability to estimate distribution ratios correctly. We consider the inner optimization for \texttt{ReCOIL-Q} :
% \begin{align}
% &\min_{Q(s,a)}  \beta (1-\gamma)\E{d_0(s),\pi(a|s)}{Q(s,a)} +\E{s,a\sim d_{mix}^{E,R}}{f^*_p( \mathcal{T}_0^\pi Q(s,a)-Q(s,a))}\nonumber \\
% &~~~~~~~~~~~~~~~~~~ - (1-\beta) \E{s,a\sim d^R}{ \mathcal{T}_0^\pi Q(s,a)-Q(s,a)}
% \end{align}
% The following holds for the inner optimization for \texttt{ReCOIL-Q} when $Q$ is optimized (see Appendix~\ref{ap:closer} for the proof):
% \begin{equation}
%     f^{*^'}_p(\mathcal{T}_0^\pi Q(s,a)-Q(s,a))=\frac{\beta d^\pi(s,a) + (1-\beta)d^R(s,a)}{\beta d^E(s,a)+(1-\beta)d^R(s,a)}.
%     \label{eq:mixture_density_ratio}
% \end{equation}
% Thus, given the visitation distribution of the replay buffer $d^R$, expert $d^E$ and the policy $\pi$, the inner optimization implicitly learns the distribution ratio in Eq~\ref{eq:mixture_density_ratio}, allowing us to infer agent visitation $d^\pi$. This estimation is at the heart of all dual-RL methods and allows for off-policy evaluation -- which requires inferring $d^\pi$, off-policy optimization where we are interested in figuring out current policy visitation $d^\pi$ in order to improve it, and imitation learning where we are interested in the ratio $d^\pi/d^E$ in order to bring the agent closer to the expert. 
% %%AZ.2.15: Something about this sentence is off, can you re-read and rephrase?

% We consider two settings in our experiments: (1) a 2-timestep MDP (Fig~\ref{fig:distribution_ratio_estimation1}) where the agent starts from state $s_0$ and transitions to one of the states $\{s_1,s_2,s_3,s_4,s_5\}$ which are absorbing. In this setting, the replay buffer perfectly covers the unknown ground truth agent visitation. (2) a 2-D gridworld (Fig~\ref{fig:distribution_ratio_estimation2}) where the agent can move cardinally and the replay buffer distribution does not cover the unknown ground truth agent visitation. 
% \begin{figure}[h]
% \begin{center}
% \includegraphics[width=0.9\linewidth]{figures/density_ratio_estimation/perfect_coverage_1d.pdf}
%       \\
%       \vspace{-2.0mm}
% \end{center}
% % \vspace{-1.0mm}
% \caption{The replay buffer distribution covers the agent policy visitation distribution. Using \texttt{ReCOIL}, we are perfectly able to infer the agent policy visitation whereas a method that only relies on expert data or the replay data with the coverage assumption fails. Results are averaged over 100 seeds.}
% \label{fig:distribution_ratio_estimation1}
% \end{figure}
% Our results (Figure~\ref{fig:distribution_ratio_estimation1} and \ref{fig:distribution_ratio_estimation2}) demonstrate that in the perfect coverage setting, \texttt{ReCOIL} is able to infer the agent policy visitation perfectly, and in the case of imperfect coverage is able to significantly outperform other methods (IQLearn and SMODICE). Note that we modify SMODICE to incorporate state-action expert data rather than relying on state-only expert data. IQLearn does not leverage replay data information, relying only on expert data to infer agent visitation. SMODICE's reward function $-\log \frac{d^R(s,a)}{d^E(s,a)}$, arising from its coverage assumption is ill-defined in parts of state space where the expert has no support leading to poor downstream density ratio estimation.


% \begin{figure}[h]
% \begin{center}
%     \includegraphics[width=0.9\linewidth]{figures/density_ratio_estimation/imperfect_coverage_2d.pdf}
%       \\
%       \vspace{-2.0mm}
% \end{center}
% % \vspace{-1.0mm}
% \caption{Replay buffer consists of data that visits near the initial state (0,0), a setting commonly observed when training RL agents. We estimate agent's policy visitation and observe \texttt{ReCOIL} to outperform both methods which rely on expert data only or use the replay data with coverage assumption}
% \label{fig:distribution_ratio_estimation2}
% % \vspace{-0.8mm}
% \end{figure}
\subsection{Offline RL}

\begin{wrapfigure}{r}{0.4\textwidth}
\vspace{-35pt}
\begin{center}
\includegraphics[width=1.0\linewidth]{figures/offline_rl_analysis/xql++analysis.pdf}
      \\
      \vspace{-2.0mm}
\includegraphics[width=1.0\linewidth]{figures/offline_rl_analysis/xql++analysis_legend.pdf}  
    \vspace{-7.5mm}
\end{center}
\caption{XQL training diverges due to the numerical instability of its loss function. $f$-DVL fixes this problem by using dual of more well-behaved $f$-divergences.}
% \qq{change plot legend}}
% \vspace{-5pt}
\label{fig:offline-rl-analysis}
% \vspace{-0.8mm}
\end{wrapfigure}

\textbf{Benchmark and Analysis.}
On a broad range of continuous control tasks in offline RL from the D4RL benchmarks~\cite{fu2020d4rl}, $f$-\texttt{DVL} outperforms XQL and other prior methods~\citep{chen2021decision,kumar2019stabilizing,kumar2020conservative,kostrikov2021offline,fujimoto2021minimalist}. We note an inconsistency in the XQL results with fixed hyperparameters: their results were reported by taking the best average return during training as opposed to the standard practice of taking the average of the last iterate performance across different seeds at 1 million gradient steps. This inconsistency can be validated by comparing their training plots and reported results (Fig 11 and Table 1 in  \cite{garg2023extreme}). XQL(r) shows the results for XQL with the standard evaluation protocol using the author's implementation under the same hyperparameters. 


\begin{table}[t]
\vspace{-10pt}
\centering
\scriptsize
\setlength\tabcolsep{3pt}
\renewcommand{\arraystretch}{1.0}
% \vspace{-0.1in}
% \vspace{5pt}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l||rrrrrrr|cc}
% \parbox[t]{2mm}{\multirow{9}{*}{\pix\rotatebox[origin=c]{90}{\textbf{Online} \hspace{2.5em}}}} 
% & 
\multicolumn{1}{c||}{Dataset} & BC & 10\%BC & DT  & TD3+BC & CQL & IQL &  {XQL}(r) & \bf{$f$-DVL} ($\chi^2$) & \bf{$f$-DVL} (TV)\\\hline
% \parbox[t]{2mm}{\multirow{9}{*}{\pix\rotatebox[origin=c]{90}{\textbf{Gym}}}} 
% & ~~ 
halfcheetah-medium-v2 & 42.6 & 42.5 & 42.6  & \highlight{48.3} &44.0 & \highlight{47.4} & 47.4 & \highlight{47.7} & 47.5\\ 
% & ~~ 
hopper-medium-v2 & 52.9 & 56.9 & 67.6 &  59.3 & 58.5 & 66.3  & \highlight{68.5} & 63.0& 64.1\\ 
% &~~ 
walker2d-medium-v2 & 75.3 &75.0 &74.0 & \highlight{83.7} & 72.5 & 78.3  & 81.4 & 80.0 & 81.5\\ 
% & ~~ 
halfcheetah-medium-replay-v2 & 36.6 & 40.6 & 36.6 &  \highlight{44.6} & \highlight{45.5} &\highlight{ 44.2}  &44.1  & 42.9 & \highlight{44.7}\\ 
% % & ~~ 
hopper-medium-replay-v2 & 18.1 & 75.9 & 82.7 & 60.9 & 95.0 &  94.7  &95.1  & 90.7&\highlight{98.0}\\ 
% & ~~ 
walker2d-medium-replay-v2 & 26.0 & 62.5 & 66.6 &  \highlight{81.8} & 77.2 & 73.9  &58.0 &52.1&68.7  \\ 
% & ~~ 
halfcheetah-medium-expert-v2 & 55.2 & \highlight{92.9} & 86.8 &   90.7 & \highlight{91.6} & 86.7 &  90.8 &89.3 &\highlight{91.2} \\ 
% & ~~ 
hopper-medium-expert-v2 &52.5 & 110.9 & \highlight{107.6}  & 98.0 & 105.4 & 91.5  & 94.0 &\highlight{105.8} & 93.3 \\ 
% & ~~ 
walker2d-medium-expert-v2 & 107.5 & \highlight{109.0} & 108.1  & \highlight{110.1} & 108.8 & \highlight{109.6}  & \highlight{110.1} &\highlight{110.1} & 109.6\\ \hline 
% locomotion-v2 total & 466.7 & 666.2 & 672.6 & 450.7 & 684.6 & 677.4 & 698.5 & 692.4 & --\\ \hline
% \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{AntMaze}}}} 
% & ~~ 
antmaze-umaze-v0 & 54.6 & 62.8 & 59.2 & 78.6 & 74.0 & \highlight{87.5}  & 47.7&83.7 &\highlight{87.7} \\ 
% & ~~ 
antmaze-umaze-diverse-v0 & 45.6 & 50.2 & 53.0 &  71.4 & \highlight{84.0} & 62.2  & 51.7   &  50.4&48.4\\  
% & ~~ 
antmaze-medium-play-v0 & 0.0 & 5.4 & 0.0 &  10.6 & 61.2 & \highlight{71.2}  &  31.2 & 56.7&\highlight{71.0} \\  
% & ~~
antmaze-medium-diverse-v0 & 0.0 & 9.8 & 0.0 &  3.0 & 53.7 & \highlight{70.0}  &  0.0& 48.2& 60.2\\  
% & ~~ 
antmaze-large-play-v0 &0.0 &0.0 &0.0 &0.2 &15.8 & 39.6  &10.7 &36.0 & \highlight{41.7}\\  
% & ~~ 
antmaze-large-diverse-v0 & 0.0 &6.0 & 0.0 & 0.0 & 14.9 & \highlight{47.5} &31.28 &\highlight{44.5} & 39.3\\ \hline 
% antmaze-v0 total & 100.2 & 134.2 & 112.2 & 107.7 & 125.3 & 163.8 & 303.6 & 378.0 & -- \\
%\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{Franka}}}} 
% & ~~ 
kitchen-complete-v0 & 65.0 & -  & -  & - &43.8 & 62.5  & 56.7 &\highlight{67.5} &61.3 \\ 
% & ~~ 
kitchen-partial-v0 &38.0 & - & - & - & 49.8 & 46.3   & 48.6 &58.8 & \highlight{70.0} \\ 
% & ~~ 
kitchen-mixed-v0 & 51.5 & - & - &  - & 51.0 & 51.0 & 40.4  & \highlight{53.75}&52.5 \\ \hline \hline
% & runtime & 10m & 10m & 960m & 20m & 20m & 20m & 80m & 20m & 10-20m & 10-20m$^*$ \\
\end{tabular}
}
\caption{Averaged normalized return of offline RL methods on D4RL tasks. XQL(r) denotes the results obtained with our own implementation. Results are averaged over 7 random seeds.}
\vspace{-5pt}
\label{tab:d4rl}
\end{table}


\textbf{Analysis}: XQL's loss function contains exponential loss terms that cause numerical instability as pointed out by the authors. This loss function is the by-product of using the RKL divergence and is fixed by $f$-\texttt{DVL} by using loss functions corresponding to more stable divergences as can be seen in Fig~\ref{fig:offline-rl-analysis}. Our additional experiments for online RL in Fig.~\ref{fig:online_rl} demonstrate that  $f$-\texttt{DVL} also increases sample efficiency and training stability in the online setting as well. Additional description and implementation details as well as all the learning curves are in the Appendix~\ref{ap:additional_experiments}. 
\begin{figure*}[h]
\begin{center}
          \includegraphics[width=0.9\linewidth]{figures/online_rl/online-rl.pdf}
      \\
      \vspace{-2.0mm}
    \includegraphics[width=1.0\linewidth]{figures/online_rl/offline-rl-legend.pdf}  
    % \vspace{-8.2mm}
\end{center}
\vspace{-3.0mm}
\caption{$f$-\texttt{DVL} increases training stability and learning performance particularly in Hopper-Hop and Quadruped-Run for online RL.}
\label{fig:online_rl}
\end{figure*}


\subsection{Analyzing and Ablating dual-RL} 
We further investigate dual-RL approaches further in Appendix showing: a) how dual-RL methods are able to leverage truly off-policy data where traditional ADP methods like SAC, and TD3 fail (Appendix~\ref{}), b) the sensitivity of ReCOIL and XQL to algorithm hyperparameters (Appendix~\ref{}), c) quality of learned reward functions in ReCOIL (Appendix~\ref{}).

% Considering the breadth of the framework, we limit our experiments to a) showing the importance of true-offpolicyness afforded by the dual RL methods and answering the following questions about our proposed off-policy imitation learning method from arbitrary experience: b) Does utilizing off-policy data in the form of $f$-divergence minimization using mixture ratios allow for better estimation of the density ratio between agent and the expert? c. How well does our proposed imitation learning method perform in the offline setting when learning from diverse data and across different environments?




% \begin{table*}[h]
%     % \vspace{2mm}
%     \centering
%     \footnotesize
%     % \resizebox{\textwidth}{!}{%
%     \begin{tabular}{c|c|c|c|c|c}
%     \toprule
%     \multirow{1}{*}{Dataset} & Env & RCE & ORIL & SMODICE & ReCOIL  \\
%     \midrule
%     \multirow{3}{*}{random+expert}& hopper&51.41$\pm$38.63&73.93$\pm$11.06&\textbf{101.61$\pm$7.69}&95.04$\pm$4.48\\
%     & halfcheetah&64.19$\pm$11.06&60.49$\pm$3.53& 80.16$\pm$7.30&\textbf{84.10$\pm$4.72}\\
%     & walker2d&20.90$\pm$26.80&2.86$\pm$3.39&\textbf{105.86$\pm$3.47}&100.84$\pm$6.34\\
%     & ant&105.38$\pm$14.15&73.67$\pm$12.69&\textbf{126.78$\pm$5.12}&\textbf{126.74$\pm$4.63}\\
%     \midrule
%         \multirow{3}{*}{random+few-expert}& hopper&25.31$\pm$18.97&42.04$\pm$13.76&60.11$\pm$18.28&\textbf{79.44$\pm$13.53}\\
%     & halfcheetah& 2.99$\pm$1.07&2.84$\pm$5.52& 2.28$\pm$0.62& \textbf{3.90$\pm$0.66}\\
%     & walker2d&40.49$\pm$26.52& 3.22$\pm$3.29&\textbf{107.18$\pm$1.87}&83.23$\pm$19.00\\
%     & ant&67.62$\pm$15.81&25.41 $\pm$ 8.58&-6.10$\pm$7.85&\textbf{94.25$\pm$ 8.30}\\
%     \midrule
%     \multirow{3}{*}{medium+expert}& hopper&29.37$\pm$3.39&61.35$\pm$7.91&54.77$\pm$6.2&\textbf{63.26$\pm$4.99}\\
%     & halfcheetah&61.14$\pm$18.31& 57.15$\pm$3.49&58.01$\pm$3.12&\textbf{84.01$\pm$3.40}\\
%     & walker2d&19.84$\pm$2.71&4.14$\pm$2.69&1.2$\pm$1.57&\textbf{91.51$\pm$16.50}\\
%     & ant&81.18$\pm$29.73&103.42$\pm$8.43&102.82$\pm$4.63&\textbf{119.94$\pm$4.52} \\
%     \bottomrule
%     \end{tabular}
% \caption{Normalized scores for \texttt{ReCOIL} on the different D4RL datasets along with 1000 given expert transitions compared to different offline IL baselines. \texttt{ReCOIL} improves over baselines when the offline dataset has low coverage of expert or when it is more challenging to distinguish expert vs suboptimal transitions. } 
% \label{table:offline_rl_results}
% \end{table*}


% \begin{figure}[h]
% \begin{center}
%     \includegraphics[width=0.9\linewidth]{figures/offline_il/offline-il-coverage.pdf}
%       \\
%     \includegraphics[width=0.9\linewidth]{figures/offline_il/offline-il.pdf}
%       \\
%        \includegraphics[width=0.9\linewidth]{figures/offline_il/offline-il-legend.pdf}
%       \vspace{-2.0mm}
% \end{center}
% % \vspace{-1.0mm}
% \caption{ReCOIL performs competitively in the setting of learning to imitate from diverse offline data. The results are averaged over 5 seeds.}
% \label{fig:offline_il}
% % \vspace{-0.8mm}
% \end{figure}

==> comparison_table_with_citations.tex <==


\begin{table*}[t]
\vspace{-10pt}
% \begin{adjustbox}{max width=\textwidth}
    \centering
    \large
%    \scalebox{0.7}{
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|cccccc} 
    \toprule
    &\multicolumn{1}{c}{\textbf{Dual RL Method}}  & \textbf{Gradient} & {\textbf{Objective}}  & \textbf{dual-Q/V}& \textbf{Off-Policy Data}& \textbf{Coverage Assumption} \\
    \midrule
     % &\multirow{2}{*}{\xmark} & \multirow{2}{*}{LfD}& \multirow{2}{*}{supremum}& \multirow{2}{*}{non-linear} & \multirow{2}{*}{\xmark} \\ 
    % GCL~\cite{finn2016guided} & $\tau$ & Forward Kullback-Leibler & \checkmark  \\
    \vspace{0.5mm}    
    \multirow{4}{*}{RL}& AlgaeDICE~\cite{nachum2019algaedice}, GenDICE~\cite{zhang2020gendice}, CQL~\cite{kumar2020conservative}  &  semi  & reg. RL & $Q$ &  Arbitrary &---\\
    & OptiDICE~\cite{lee2021optidice}  & full  & reg. RL & $V$  & Arbitrary &---\\
     & XQL~\cite{garg2023extreme}, REPS~\cite{peters2010relative}, $f$-\textbf{DVL} &  semi  & reg. RL &$V$ &  Arbitrary&--- \\
      & VIP~\cite{ma2022vip}, GoFAR~\cite{ma2022far} &  full  & reg. RL & $V$ &  Arbitrary&--- \\
    &Logistic Q-learning~\cite{bas2021logistic}  & full   & reg. RL & $QV$\footnotemark[1] &  \xmark & ---\\
     \midrule
     \multirow{9}{*}{IL}& IQLearn~\cite{garg2021iq}, IBC~\cite{florence2022implicit}  & semi  & $D_f(\rho^\pi\|\rho^E)$ & $Q$ &  Expert-only & \xmark   \\
    & \textbf{IVLearn}  &  semi  & $D_f(\rho^\pi\|\rho^E)$ & $V$  & Expert-only  & \xmark \\
    & OPOLO~\cite{zhu2020off}, OPIRL~\cite{hoshino2022opirl}  & semi & $D_{rkl}(\rho^\pi\|\rho^E)$ & $Q$  & Arbitrary &  \cmark \\
    & ValueDICE~\cite{kostrikov2019imitation}  & semi & $D_{rkl}(\rho^\pi\|\rho^E)$ & $Q$  & Arbitrary &  \cmark \\
    & SMODICE~\cite{ma2022smodice} & full & $D_{rkl}(\rho^\pi\|\rho^E)$& $V$  & Arbitrary &  \cmark \\
    & DemoDICE~\cite{kim2022demodice}, LobsDICE~\cite{kim2022lobsdice}  & full & $D_{rkl}(\rho^\pi\|\rho^E)+\alpha D_{rkl}(\rho^\pi\|\rho^R) $& $V$  & Arbitrary &  \cmark \\
     & P$^2$IL~\cite{viano2022proximal} & full & $D_{C}(\rho^\pi\|\rho^E)$\footnotemark[1] & $QV$\footnotemark[1]  &\xmark & \xmark  \\
    & \textbf{ReCOIL-Q}  & full & $D_{f}(\rho^\pi_{mix}\|\rho^{E,R}_{mix})$& $Q$ &   Arbitrary &  \xmark \\[0.1cm] 
    & \textbf{ReCOIL-V}   & full & $D_{f}(\rho^\pi_{mix}\|\rho^{E,R}_{mix})$& $V$ &   Arbitrary &  \xmark \\
    \bottomrule
    \end{tabular}
    % \end{adjustbox}
    }
    \vspace{-5pt}
    %%AZ.5.16: You still don't refer to this table anywhere.
    \caption{A number of recent works can be studied together under the unified umbrella of \textbf{dual-RL}. These methods are instantiations of dual-RL with a choice of update strategy, objective, constraints, and their ability to handle off-policy data. \textbf{Bold} names correspond to the methods proposed in the paper.}
    \label{tab:works}
    % \vspace{-7mm}
\end{table*}
\footnotetext[1]{These methods use a different regularizer. More details in Appendix~\ref{ap:LQL_P2IL}.}


==> recoil-proof-old.tex <==
ReCOIL optimizes the lagrangian dual for the following primal:
\begin{align}
    &\max_{d(s,a)\ge0,\pi(a|s)} -\f{d^R_\text{mix}(s,a)}{d^{E,R}_\text{mix}(s,a)} \nonumber\\
    &\text{s.t}~~\sum_a d(s,a)=(1-\gamma)\rho_0(s)+\gamma \sum_{s',a'} d(s',a')p(s|s',a').
\end{align}

It is not directly clear how simply replacing the objective from matching agent's visitation density with expert's density to matching mixture distribution allows ReCOIL to exploit off-policy data to improve learning performance. We explain why this is step-by-step in the section below:

\subsubsection{How does ReCOIL exploit off-policy data to improve performance?}
\qq{gap(importance sampling when $d \in D_\delta$) + gap(any $d$ and $d \in D_\delta$).}

\qq{I think it's better to emphasize that the approximation of $\E{d}{\gamma V(s')-V(s)}$
by $\E{d^E}{\frac{d(s,a)}{d^E(s,a)}(\gamma V(s')-V(s))}$ might be inexact, since $d^E$ and $d$ might have different
support, and we analyze the approximation error introduced by importance sampling without making any assumptions.
}



We consider the empirical suboptimal dataset of transitions given by $d^S$ and also the empirical expert visitation distribution given by $d^{\hat{E}}$. We distinguish $d^{\hat{E}}$ from $d^{E}$ to stress that the dataset might not cover the true expert distribution completely. A reasonable guarantee to achieve when optimizing a policy in the dataset is to find a policy that stays in support of this seen dataset $D=d^S\cup d^{\hat{E}}$ of transitions while being the closest to the expert. \qq{I think you're mixing two concepts here: datasets and distribution} We define a set of all visitation distributions $D_\delta$ such that any visitation from this set has a probability mass of $1-\delta$ in the joint support of $d^S\cup d^{\hat{E}}$, i.e $\int d(s,a) \mathbbm{1}(d^S>0 ~\text{or}~d^{\hat{E}}>0) \ge 1-\delta$ \qq{$\Pr_d((s,a) \in S^J) \geq 1 -\delta.$ use $S$ for support, $d$ for distribution.}. 
\hs{replace E BY $\hat{E}$} \qq{I'm not sure whey you need $\hat{E}$. the rest should work for $d^E$ as well, right?}
The imitation objective in its lagrangian formulation takes the following form by replacing $d^O=d^E$ for \primalV:

\begin{equation}
\label{eq:original_objective_imitation}
    \min_V \max_{d \in D} (1-\gamma)\E{d_0(s)}{V(s)} + \E{d}{\gamma V(s')-V(s)} -\f{d}{d^E} 
\end{equation}

To get an analytical closed form for the inner maximization, the derivation for \texttt{IV-Learn} relies on importance sampling:
\begin{equation}
\label{eq:ivlearn_objective_imitation}
    \min_V \max_{d \in D} (1-\gamma)\E{d_0(s)}{V(s)} + \E{d^E}{\frac{d(s,a)}{d^E(s,a)}(\gamma V(s')-V(s))} -\E{d^E}{f\left(\frac{d(s,a)}{d^E(s,a)}\right)} 
\end{equation}


For ReCOIL, the objective considers the mixture distribution regularization and the Lagrangian dual takes the following form:

\begin{align}
\label{eq:recoil_objective_imitation}
\min_V \max_{d \in D} \beta(1-\gamma)\E{d_0(s)}{V(s)} + \E{s,a\sim \dmix}{\gamma V(s')-V(s)} - \f{\dmix}{\demix} \nonumber\\ - (1-\beta) \E{d^S}{\gamma V(s')-V(s)}
\end{align}
To get an analytical solution for inner optimization we use importance sampling to derive \texttt{ReCOIL}:

\begin{align}
\min_V \max_{d \in D} \beta(1-\gamma)\E{d_0(s)}{V(s)} + \E{s,a\sim \demix}{\frac{\dmix}{\demix}(\gamma V(s')-V(s))} - \E{\demix}{f\left(\frac{\dmix}{\demix}\right)} \nonumber \\- (1-\beta) \E{d^S}{\gamma V(s')-V(s)}
\end{align}
which can be further simplified to
\begin{align}
\min_V \max_{d \in D} \beta(1-\gamma)\E{d_0(s)}{V(s)} + \beta\E{s,a\sim \demix}{\frac{d(s,a)}{\demix}(\gamma V(s')-V(s))} - \E{\dmix}{f\left(\frac{\dmix}{\demix}\right)} 
\end{align}
\qq{is the last term's expectation right? should be $d^{E,S}$?}

To simplify the analysis, we consider the case when mixture ratio $\beta \to 1$, and focus on the quantity that we are trying to estimate via importance sampling: $\E{d(s,a)}{\gamma V(s')-V(s)}$. Under the visitation distribution set $D_\delta$ (note $D=D_{\delta=0}$), IV-Learn's objective suffers from the following worst-case estimation error due to the importance sampling step $\forall~~d\in D_{\delta=0}$ \qq{need to explain $\gamma V(s') - V(s) \geq 0, \forall s \in \S$}:
\begin{align}
    \E{d}{(\gamma V(s')-V(s))}-\E{d^E}{\frac{d(s,a)}{d^E(s,a)}(\gamma V(s')-V(s))} &\le \E{d}{(\gamma V(s')-V(s))}\\
    &\le \max \gamma V(s') - V(s) \le R_{\max}
\end{align}

{
\color{red}
This holds for any $d$
\begin{align}
    \E{d}{(\gamma V(s')-V(s))}-\E{d^E}{\frac{d(s,a)}{d^E(s,a)}(\gamma V(s')-V(s))} & \leq \E{(s,a) \in S^d \backslash S^E}{(\gamma V(s')-V(s))}\\
    &\le \max \gamma V(s') - V(s) \le R_{\max}
\end{align}
where $S^E$ is the support of .... 
}



The first term above is the oracle estimation of the quantity of interest for any $d\in D_{\delta=0}$ and the second is the estimate of the same quanity using importance sampling with $d^E$.

Compared to IV-Learn, ReCOIL can leverage offline dataset to improve estimation accuracy of the training objective as follows:
\begin{align}
    \E{d}{(\gamma V(s')-V(s))}-\E{d^{E,R}_\text{mix}}{\frac{d(s,a)}{{d^{E,R}_\text{mix}(s,a)}}(\gamma V(s')-V(s))} \le \E{ s,a \notin S^J}{(\gamma V(s')-V(s))} \nonumber \\
    \le \max \delta (\gamma V(s') - V(s)) \le \delta R_{\max}
\end{align}

{
\color{red}
This holds for $d \in D_\delta$
\begin{align}
    \E{d}{(\gamma V(s')-V(s))}-\E{d^{E,R}_\text{mix}}{\frac{d(s,a)}{{d^{E,R}_\text{mix}(s,a)}}(\gamma V(s')-V(s))} \leq \E{ s,a \in S^d \backslash S^J}{(\gamma V(s')-V(s))} \nonumber \\
    \le \max \delta (\gamma V(s') - V(s)) \le \delta R_{\max}
\end{align}

}

The second line above follows due to the assumption that and $d$ in $D_{\delta}$ has $1-\delta$ probability mass in the support of $D$. We refer to the error in estimating the quantity $\E{d}{(\gamma V(s')-V(s))}$ using some off-policy data as the estimation or the approximation error.


\subsubsection{Estimation/Approximation error to Performance bound \hs{change}}


% \begin{center}
%     \begin{tabular}{ |c|c|c|c| } 
%     \hline
%     Divergence & $f$ & $\kappa$ & Domain \\
%      \hline
%      \hline
%      relative entropy (KL) & $ t \log t $ & $\frac 1 M$ & $(0,M]$ \\
%      \hline
%      total variation & $\frac{|t-1|}{2}$ & $0$ & $(0,\infty)$ \\
%      \hline
%      Pearson's $\chi^2$& $(t-1)^2$ & $2$ & $(0,\infty)$\\ 
%      \hline
%      squared Hellinger & $2( 1 - \sqrt{t} ) $& $M^{- \frac 3 2}/2$ & $(0,M]$\\ 
%      \hline
%      reverse relative entropy & $-\log t$ & $1/M^2$ & $(0,M]$\\ 
%      \hline
%      Vincze- Le Cam & $\frac{(t-1)^2}{t+1}$ & $\frac{8}{ (M+1)^3}$ & $(0, M]$ \\
%      \hline
%      Jensen-Shannon & $(t+1)\log \frac{2}{t+1} + t \log t$ & $\frac{1}{M(M+1)}$ & $(0,M]$ \\
%      \hline
%      Neyman's $\chi^2$ & $\frac 1 t - 1$ & $2/M^3$ & $(0,M]$ \\
%      \hline
%      Sason's $s$ & $\log(s+t)^{(s+t)^2 } -  \log(s+1)^{(s+1)^2}$ & $2 \log(s + M) + 3$ & $[M,\infty)$, $s > e^{-3/2}$\\
%      \hline
%      $\alpha$-divergence & $\frac{4\left( 1- t^{\frac{1 + \alpha}{2}}\right)}{1-\alpha^2}, \hspace{2mm} \alpha \neq \pm 1$ & $M^{\frac{\alpha - 3}{2}}$ & $ \begin{cases}
%          [M,\infty), \hspace{2mm} \alpha > 3 \\
%             (0, M], \hspace{2mm} \alpha < 3
%      \end{cases}$ \\  
%      \hline
    
%     \end{tabular}   
%     \end{center}

% \end{table}

In the offline setting, akin to pessimism principle in offline RL, we aim to return the closest-to-expert in-dataset policy. We will see that \texttt{ReCOIL}-V can naturally incorporate such pessimism using implicit maximization. Assuming that \texttt{ReCOIL} can enforce this constraint approximately (searches for a policy visitation within $D_\delta$), we derive its performance error. For ease of notation we denote the oracle objective which searches for visitations within $D$ in Eq.~\eqref{eq:recoil_objective_imitation} as $\min_V \max_d g(d,V)$ and the realistic objective which searches for visitations within $D_\delta$ in Eq.~\eqref{eq:recoil_objective_imitation} as $\min_V \max_d \hat{g}(d,V)$. Let the gap between these two objectives is given to be upper bounded by an approximation error denoted by $\epsilon_\text{approx}$. \qq{I think there shouldn't be $D$? only needs $D_\delta$}
% For ease of notation, let's denote our original objective to be optimized for imitation given by Eq.~\eqref{eq:original_objective_imitation} as $\min_V \max_d g(d,V)$ and the estimated objectives given by Eq.~\eqref{eq:ivlearn_objective_imitation} or Eq.~\eqref{eq:recoil_objective_imitation} as $\hat{g}(d,V)$. 
\begin{equation}
\label{eq:bounded_approx_error}
    |g(d,V)-\hat{g}(d,V)|\le \epsilon_\text{approx}
\end{equation}

{
\color{red}
\begin{equation}
    \max_{d, V}|g(d,V)-\hat{g}(d,V)|\le \epsilon_\text{approx}
\end{equation}
}

Further let $\max_d \hat{g}(d,V) = \hat{h}(V)$ and $\max_d g(d,V) = h(V)$. It follows that: $|\hat{h}(V)-h(V)|\le 2\epsilon_\text{approx}$ which directly follows from Eq.~\eqref{eq:bounded_approx_error}. 

We now show that $h$ and $\hat{h}$ are convex functions in $V$ as follows:
First, recall definition of $\hat{h}(V)$
\begin{align}
\hat{h}(V) = \min_V \max_d \beta(1-\gamma)\E{d_0(s)}{V(s)} + \E{s,a\sim d^{E,R}_\text{mix}}{\frac{d^{R}_\text{mix}(s,a)}{d^{E,R}_\text{mix}(s,a)}(\gamma V(s')-V(s))} - \E{d^{E,R}_\text{mix}}{f\left(\frac{d^R_\text{mix}(s,a)}{d^{E,R}_\text{mix}(s,a)}\right)} \nonumber \\- (1-\beta) \E{d^R}{\gamma V(s')-V(s)}
\end{align}
which can be simplified using a closed form solution for inner maximization:
\begin{align}
\hat{h}(V) = \min_V  \beta(1-\gamma)\E{d_0(s)}{V(s)} + \E{s,a\sim d^{E,R}_\text{mix}}{f^*_p(\gamma V(s')-V(s))} - (1-\beta) \E{d^R}{\gamma V(s')-V(s)}
\end{align}
The first and last term above are linear in $V$ and all that remains is to show strong convexity for the function $f^*_p(\gamma V(s')-V(s))$. We demonstrate that below:
\begin{align}
    f^*_p(x) := -f\Big(\max\Big(0, (f')^{-1}(x) \Big) \Big) + \max \Big(0,  (f')^{-1}(x) \Big)\cdot x.
\end{align}
 $f^*_p(x)$ can be shown to be convex in $x$ by showing ${f^*_p}''(x) \ge 0~\forall x$. Note that $f'$ is a strictly increasing function by the strict convexity of $f$, which implies that $(f')^{-1}$ is also a strictly increasing function.,
\begin{align*}
    f^*_p(x) &= -f( (f')^{-1}(x) ) + (f')^{-1}(x) \cdot x, \\
    {f^*_p}'(x) &= -x \cdot  ((f')^{-1})'(x) + ((f')^{-1})'(x) \cdot x + (f')^{-1}(x) \\
          &= (f')^{-1}(x), \\
    {f^*_p}''(x) &= ((f')^{-1})'(x),
    %~~~ \text{($\because$ the derivative of the strictly increasing function $(f')^{-1}$)}
\end{align*}
where $((f')^{-1})'(x) > 0$ since it is the derivative of the strictly increasing function $(f')^{-1}$. We also note that $h$ and $\hat{h}$ is  $\kappa$-strongly convex with  $\kappa$  given in Table~\ref{tab:strong_convexity}.
\newline
\begin{table}[h]
\begin{center}
    \begin{tabular}{ |c|c|c|c| } 
    \hline
    Divergence & $h''(x)={f*}^{''}(x)$ & $\kappa$ & Domain \\
     \hline
     \hline
     Forward (KL) & $ \frac{1}{x^2} $ & $\frac{1}{M^2}$ & $(0,M]$ \\
     \hline
     total variation & 0 & 0 & $(0,\infty)$ \\
     \hline
     Pearson's $\chi^2$& $\frac{1}{2}$ & $0.5$ & $(0,\infty)$\\ 
     \hline
     Reverse KL & $e^{x-1}$ & $e^{-1}$ & $(0,M]$\\ 
     \hline
    
    \end{tabular}   
    \end{center}
\caption{Table shows values of $\kappa$ where a divergence generator $h$ is $\kappa$ strongly convex on the Domain.[\cite{melbourne2020strongly}]}
\label{tab:strong_convexity}
\end{table}
Now we are interested in finding an upper bound to the following to be able to comment how far the value function obtained via approximate objective is compared to the true optimal value function:
\begin{align}
\label{eq:to_be_upper_bounded}
    \min_V \hat{h}(V) - \min_V h(V) 
\end{align}


Let $\hat{V} = \argmin_V \hat{h}(V)$ and $\argmin_V h(V) = V^* $. Then we can rewrite Eq.~\eqref{eq:to_be_upper_bounded} and further simplify it:
\hs{QQ review and HS review: Absolute bound proof does not hold}


\begin{align}
\label{eq:upper_bounded_to_objective_mismatch}
    \hat{h}(\hat{V}) - h(V^*) &= \hat{h}(\hat{V})-\hat{h}(V^*) +\hat{h}(V^*) - h(V^*)\\
    &\le \hat{h}(V^*) - h(V^*)\\
    & \le 2\epsilon_\text{approx} 
\end{align}



% \begin{align}
% \label{eq:lower_bounded2_to_objective_mismatch}
%      h(V^*) - \hat{h}(\hat{V}) &= \hat{h}(\hat{V})-h(\hat{V}) +h(\hat{V}) - h(V^*)\\
%     &\ge \hat{h}(V^*) - h(V^*)\\
%     & \ge \epsilon_\text{approx}
% \end{align}

% \begin{align}
%     \label{eq:upper_bounded_to_objective_mismatch}
%     |\hat{h}(\hat{V}) - h(V^*)| &= |\hat{h}(\hat{V})-\hat{h}(V^*) +\hat{h}(V^*) - h(V^*)|\\
%     &\le |\hat{h}(V^*) - h(V^*)|\\
%     & \le \epsilon_\text{approx}
% \end{align}

The second step follows because $\hat{h}(\hat{V})-\hat{h}(V^*)\le 0$ as $\hat{h}(\hat{V})$ is the minimum value for $\hat{h}$. We also have the following relation from Eq.~\eqref{eq:to_be_upper_bounded}:
\begin{align}
    \label{eq:lower_bounded_to_objective_mismatch}
   %  \hat{h}(\hat{V}) - h(V^*) \ge  h(\hat{V}) - h(V^*)  \geq- 2\epsilon_\text{approx}
    \hat{h}(\hat{V}) - h(V^*)  =  \hat{h}(\hat{V})- h(\hat{V}) + h(\hat{V}) - h(V^*) \geq -2\epsilon_\text{approx}.
\end{align}
Combining the above two equations Eq.~\eqref{eq:lower_bounded_to_objective_mismatch} and Eq.~\eqref{eq:upper_bounded_to_objective_mismatch}, we get:
\begin{align}
    h(\hat{V}) - h(V^*) \le 4\epsilon_\text{approx}.
\end{align}
Now, we can leverage the fact that $h$ is $\kappa$-strongly convex to further simplify the above equation:
\hs{change to frobenius norm notation}
\qq{rewrite in one big inequality: $4\epsilon_\text{approx} \geq \ldots \geq \ldots$}
\begin{align}
    h(\hat{V}) - h(V^*) &\le 4\epsilon_\text{approx}\\
    h(V^*) + (V^*-\hat{V})\nabla h(V^*) + \frac{\kappa}{2}\|V^*-\hat{V}\|^2_2 - h(V^*) &\le 4\epsilon_\text{approx}\\
    \frac{\kappa}{2}\|V^*-\hat{V}\|^2_2  &\le 4\epsilon_\text{approx}\\
    \|V^*-\hat{V}\|^2_2 &\le \frac{8\epsilon_\text{approx}}{\kappa}\\
    \|V^*-\hat{V}\|_2 &\le 2\sqrt{\frac{2\epsilon_\text{approx}}{\kappa}}\\
    \|V^*-\hat{V}\|_\infty &\le 2\sqrt{\frac{2\epsilon_\text{approx}}{\kappa}}
\end{align}

The second equation above follows as a result of strong convexity. The above derivation bounds the value function obtained ($\hat{V}$) through an approximate/estimated objective function compared to the value function obtained from the true objective ($V^*$). For an expert reward function: $R^{E}\in[0,1]$, without loss of generality, we can use~\cite{singh1994upper} to obtain the performance gap of the policies that follow these obtained value function greedily. Let $\pi_V$ denote a policy $\pi$ that acts greedily with value function $V$ then,

\begin{equation}
    J^{\pi_{V^*}}-J^{\pi_{\hat{V}}}\le \frac{4}{1-\gamma} \sqrt{\frac{2\epsilon_\text{approx}}{\kappa}}.
\end{equation}

The following two result follows depending on whether we learn from expert data alone or use all suboptimal data as in \texttt{ReCOIL}:

\textbf{Learning from expert data alone:} 
\qq{clean up this part}
\begin{equation}
    J^{\pi_{V^*}}-J^{\pi_{\hat{V}}}\le \frac{4}{1-\gamma} \sqrt{\frac{2R_{\max}}{\kappa}}
\end{equation}



% \recoil*


$$\forall \pi, \int_s d^\pi(s) \mathbf{1}_{d^O(s) > 0 \text{\, or \, } d^E(s) > 0} \geq 1 -\delta.$$

$$ \pi^1 = \argmax_{\pi} \mathbb{E}_{s} V^\pi(s), \, \text{s.t.} d^\pi(s) = 0, \, \forall d^O(s) = 0$$

$$ \pi^1 = \argmax_{\pi} \mathbb{E}_{s \sim d^O} V^\pi(s)$$

\textbf{Learning from expert data + suboptimal data as in \texttt{ReCOIL}:} 

\begin{equation}
    J^{\pi_{V^*}}-J^{\pi_{\hat{V}}}\le \frac{4}{1-\gamma} \sqrt{\frac{2\delta R_{\max}}{\kappa}}
\end{equation}


The above results demonstrate that \texttt{ReCOIL} is able to leverage suboptimal data with an approximate in-distribution policy improvement and results in a policy close to the best policy with visitation in-support of the dataset.


% The importance sampling distribution we use for IV-Learn and ReCOIL affects their estimation error in the optimization objective. We are interested to study how this error affects the downstream policy performance.

% \begin{equation}
%     \min_V \max_d \hat{g}(d,V) 
% \end{equation}
% where $\hat{g}(d,V)$ is given by either Eq.~\eqref{} or Eq.~\eqref{}. First, we note that the inner maximization is concave w.r.t d. \hs{Add proof}. Thus for any V, the inner maximization can have an error of at most the approximation error. Formally, we optimize,
% \begin{equation}
%     \min_V \hat{g}(\hat{d}(V),V)
% \end{equation}
% where $\hat{d}(V)=\argmax_d \hat{g}(d,V)$. It also follows that $\|\hat{g}(\hat{d}(V),V)- g(d^*(V),V)\|\le \epsilon_\text{approx},~~\forall V$ and susequently $\|\hat{g}(\hat{d}(V),V)- \hat{g}(d^*(V),V)\|\le 2\epsilon_\text{approx},~~\forall V$. Let $\hat{h}(V)=\hat{g}(\hat{d}(V),V)$ and $h(V)=\hat{g}(d^*(V),V)$. Note that $h$ and $\hat{h}$ are convex w.r.t V with $h'(x)=\hat{h}'(x) = (1-\gamma)+{f'}^{-1}(x)$ and $h''(x)=\hat{h}''(x)=(({f'}^{-1})'(x)>0$ \hs{Add proof}. Using the upper quadratic for convex functions we get:

% \begin{align}
%     \hat{h}(V) - 
% \end{align}


